Tiresias: Online Anomaly Detection for Hierarchical Operational Network Data

Operational network data, management data such as customer care call logs and equipment system logs, is a very important source of information for network operators to detect problems in their networks. Unfortunately, there is lack of efficient tools to automatically track and detect anomalous events on operational data, causing ISP operators to rely on manual inspection of this data. While anomaly detection has been widely studied in the context of network data, operational data presents several new challenges, including the volatility and sparseness of data, and the need to perform fast detection (complicating application of schemes that require offline processing or large/stable data sets to converge). To address these challenges, we propose Tiresias, an automated approach to locating anomalous events on hierarchical operational data. Tiresias leverages the hierarchical structure of operational data to identify high-impact aggregates (e.g., locations in the network, failure modes) likely to be associated with anomalous events. To accommodate different kinds of operational network data, Tiresias consists of an online detection algorithm with low time and space complexity, while preserving high detection accuracy. We present results from two case studies using operational data collected at a large commercial IP network operated by a Tier-1 ISP: customer care call logs and set-top box crash logs. By comparing with a reference set verified by the ISP's operational group, we validate that Tiresias can achieve >94% accuracy in locating anomalies. Tiresias also discovered several previously unknown anomalies in the ISP's customer care cases, demonstrating its effectiveness.

==> proof.tex <==

%\section*{Appendix: Proof of Lemmas}\label{sec:appendix:proof}
%\section*{Appendix: Proof of Holt Winters' Linearity}\label{sec:appendix:proof}

%\begin{lem}\label{lem:shhh:uniqueness:ap}
%{\normalfont
%Given a hierarchical tree where each node $n$ is associated with a \emph{modified weight} value $W_n[k, t]$. 
%For leaf nodes, the modified weight $W_n[k, t]$ is equal to the original weight $A_n[k, t]$.
%For non-leaf (internal) nodes, the modified weight $W_n[k, t]$ is the summation of weights of its children that are themselves \emph{not} a heavy hitter, i.e., the modified weight for non-leaf nodes can be derived by
%\begin{equation*}
%W_n[k, t] = \sum_{m} W_{m}[k, t] : m \in child(n) \cap m \in \textsf{SHHH}[\theta, t]
%\end{equation*}
%and the succinct hierarchical heavy hitter set is defined by \\
%$\textsf{SHHH}[\theta, t]= \{n | W_n[k, t] \ge \theta \}$.
%Then $\textsf{SHHH}[\theta, t]$ is unique.
%}
%\proof{
%{\normalfont
%Suppose that more than one solution exists. 
%Then there must exists one node $n$ who is in one set $\textsf{SHHH}^{(1)}$ but not in another set $\textsf{SHHH}^{(2)}$.
%Then we know $W_n^{(1)} \neq W_n^{(2)}$. By definition, there must exists a node $m \in child(n)$ where $W_m^{(1)} \neq W_m^{(2)}$.
%Repeating the above procedures, we end up having a \emph{leaf} node $p$ where $W_p^{(1)} \neq W_p^{(2)}$, which violates the
%definition of the modified weight for leaf nodes.
%}}
%\end{lem}
% 
% \begin{lem}\label{lem:shhh:position:ap}
% {\normalfont For each time instance, after the adaptations we have $n.\textsf{ishh}$ iff $n \in \textsf{SHHH}$ for any node $n \in \textsf{Tree}$.}
% \proof{
% {\normalfont 
% We prove by induction on time instance. It is clear the argument will hold for the first time instance
% as there is no adaptation. Now we show the proof will hold for any time instance.
% For the ``if'' direction, suppose (by contradiction) there exists a node $n \in \textsf{SHHH}$
% such that $n.\textsf{ishh}$ is $false$. Then we have $n.\textsf{weight} < \theta$ because
% the function Update-Ishh-and-Weight() (Fig.~\ref{alg:update:ishh}) enforces $n.\textsf{ishh}$ iff $n.\textsf{weight} \ge \theta$.
% Then by the merge rules (line \textbf{22} in Fig.~\ref{alg:core} and line \textbf{1} in Fig.~\ref{alg:merge}),
% node $n$ will be merged to its parent so we have $n \notin \textsf{SHHH}$.
% The only exception is the root node $n_{\textrm{root}}$ which has no parent to merge.
% However, we check this special case (lines \textbf{24}-\textbf{25} in Fig.~\ref{alg:core}) to
% enforce $n_{\textrm{root}}.\textsf{ishh}$ iff $n_{\textrm{root}} \in \textsf{SHHH}$.
% 
% For the ``only if'' direction, suppose (by contradiction)
% there exists a node $n$ such that $n.\textsf{ishh}$ is true
% and $n \notin \textsf{SHHH}$. Similarly, we have $n.\textsf{weight} \ge \theta$.
% Because $n.\textsf{ishh}$ is true, $n.\textsf{parent}.\textsf{tosplit}$ is also
% true (by lines \textbf{13}-\textbf{17} in Fig.~\ref{alg:core}).
% We consider the following two cases. \textbf{(i)} $n.\textsf{parent}.\textsf{washh}$ is true.
% In this case, by the induction hypothesis we know
% $n.\textsf{parent}$ was in $\textsf{SHHH}$ before any adaptation in this time instance,
% and therefore $n.\textsf{parent}$ will split its time series to $n$ (line \textbf{15} in Fig.~\ref{alg:core} and
% line \textbf{2} in Fig.~\ref{alg:separation}).
% If $n$ has no child, then we have $n \in \textsf{SHHH}$.
% Otherwise, if $n$ splits its time series, there must exists a child $n_c$ such that $n_c.\textsf{weight} < \theta$.
% If there does not exist such a child $n_c$, then we have $n.\textsf{weight}=0$ which contradicts
% our previous inference $n.\textsf{weight} \ge \theta > 0$.
% Because we have $n_c.\textsf{weight} < \theta$, by the merge rules (line \textbf{22} in Fig.~\ref{alg:core} and line \textbf{1} in Fig.~\ref{alg:merge})
% $n_c$ will merge back the time series to $n$.
% Therefore, we have $n \in \textsf{SHHH}$ after the adaptation stage.
% If the time series of $n_c$ is further split into some children, similarly, there much exists a child $n_{c'}$ of $n_c$ such
% that $n_{c'}.\textsf{weight} \le n_{c}.\textsf{weight} < \theta$. Then $n_{c'}$ will merge its time series to $n_c$, and then $n_c$ will merge back to $n$.
% It is not hard to see we can apply this argument multiple times to make sure that $n \in \textsf{SHHH}$ after the adaptation stage.
% Consider another case \textbf{(ii)} $n.\textsf{parent}.\textsf{washh}$ is false. Then we have $n.\textsf{parent} \notin \textsf{SHHH}$ before
% the adaptation stage. Because $n \notin \textsf{SHHH}$, we have $n.\textsf{parent}.\textsf{weight} \ge n.\textsf{weight} \ge \theta$.
% If $n.\textsf{parent}.\textsf{parent}.\textsf{washh}$ is true, then $n.\textsf{parent}.\textsf{parent}$ will split
% its time series to $n.\textsf{parent}$, and then $n.\textsf{parent}$ will split its
% time series to $n$ such that $n \in \textsf{SHHH}$ after the adaptation. Otherwise, if $n.\textsf{parent}.\textsf{parent}.\textsf{washh}$ is false,
% we can repeatedly apply the above argument, and finally we have $n_{\textrm{root}}.\textsf{weight} \ge \theta$ and $\neg n_{\textrm{root}}.\textsf{washh}$.
% Therefore, $n_{\textrm{root}}$ was not in $\textsf{SHHH}$ before the any adaptation in this time instance, and this violates the our
% enforcement on root node (lines \textbf{24}-\textbf{25} in Fig.~\ref{alg:core}) in the previous time instance.
% This implies the induction hypothesis is false, and we reach the contradiction.~$\square$
% }
% }
% \end{lem}
% 

\begin{lem}
\label{lem:hwlinearity:ap}
%\vspace{-5pt}
\normalfont
(Holt-Winters' Linearity). 
Given $k$ Holt-Winters' forecasts $G_1[t], G_2[t], G_k[t]$, where $G_i[t] = L_i[t-1] + B_i[t-1] + S_i[t-\upsilon]$.
Consider a time series $T^{*}[t] = \sum_{i=1}^{k}T_i[t]$ and its Holt-Winters' forecast $G^{*}[t]= L^{*}[t-1] + B^{*}[t-1] + S^{*}[t-\upsilon]$. 
Then $G^{*}[t] = \sum_{i=1}^{k}G_i[t]$.
\begin{proof}
%See Appendix B.
We show $L^{*}[t] = \sum_{i=1}^{k}L_i[t]$, $B^{*}[t] = \sum_{i=1}^{k}B_i[t]$ and $S^{*}[t] = \sum_{i=1}^{k}S_i[t]$ by induction on $t$.
For the initialization, we have
\begin{eqnarray}
L^{*}[t-1] &=& \frac{1}{2\upsilon} \sum_{j=t-1}^{t-2\upsilon} T^{*}[j] \nonumber\\
           &=& \frac{1}{2\upsilon} \sum_{j=t-1}^{t-2\upsilon} \sum_{i=1}^{k} T_i[j] \nonumber\\
           &=& \sum_{i=1}^{k} \left( \frac{1}{2\upsilon} \sum_{j=t-1}^{t-2\upsilon} T_i[j] \right) \nonumber\\
           &=& \sum_{i=1}^{k} L_i[t-1] \label{equ:hw:l:init}
\end{eqnarray}
\begin{eqnarray}
B^{*}[t-1] &=& \frac{1}{2\upsilon} \left[ \left(\sum_{j=t-1}^{\upsilon} T^{*}[j] \right) -
\left(\sum_{j=t-\upsilon-1}^{2\upsilon} T^{*}[j] \right) \right] \nonumber\\
           &=& \frac{1}{2\upsilon} \left[ \left(\sum_{j=t-1}^{\upsilon} \sum_{i=1}^{k} T_i[j] \right) -
\left(\sum_{j=t-\upsilon-1}^{2\upsilon} \sum_{i=1}^{k} T_i[j] \right) \right] \nonumber\\
           &=& \sum_{i=1}^{k} \left\{ \frac{1}{2\upsilon} \left[ \left(\sum_{j=t-1}^{\upsilon} T_i[j] \right) -
\left(\sum_{j=t-\upsilon-1}^{2\upsilon} T_i[j] \right) \right] \right\} \nonumber\\
           &=& \sum_{i=1}^{k} B_i[t-1]
\end{eqnarray}
For $j=1, \dots, 2\upsilon$, we have
\begin{eqnarray}
S^{*}[t-j] &=& T^{*}[t-j] - L^{*}[t-1] \nonumber\\
           &=& \left( \sum_{i=1}^{k} T_i[t-j] \right) - \left( \sum_{i=1}^{k} L_i[t-1] \right) \textrm{~~(by~(\ref{equ:hw:l:init}))} \nonumber\\
           &=& \sum_{i=1}^{k} \left(  T_i[t-j] - L_i[t-1] \right) \nonumber\\
           &=& \sum_{i=1}^{k} S[t-j]
\end{eqnarray}
Then we have following induction hypotheses for $j = t-1, t-2, \dots, t-2\upsilon$.
\begin{eqnarray}
L^{*}[j] &=& \sum_{i=1}^{k}L_i[j] \label{equ:hw:l:ih} \\
B^{*}[j] &=& \sum_{i=1}^{k}B_i[j] \label{equ:hw:b:ih} \\
S^{*}[j] &=& \sum_{i=1}^{k}S_i[j] \label{equ:hw:s:ih}
\end{eqnarray}
Given the induction hypotheses, it suffices to prove the theorem when $j=t$.
\begin{eqnarray}
L^{*}[t] &=& \alpha (T^{*}[t] - S^{*}[t-\upsilon]) \nonumber\\
         & & + (1 - \alpha) ( L^{*}[t-1] + B^{*}[t-1] ) \nonumber\\
         &=& \alpha \left[ \left( \sum_{i=1}^{k}T_i[t] \right) - \left( \sum_{i=1}^{k}S_i[t-\upsilon] \right) \right] + \left(1 - \alpha \right) \nonumber\\
         & & \times \left[ \left( \sum_{i=1}^{k} L_i[t-1] \right) + \left( \sum_{i=1}^{k} B_i[t-1] \right) \right] 
			%\textrm{~(by~(\ref{equ:hw:l:ih}), (\ref{equ:hw:b:ih}), (\ref{equ:hw:s:ih}))} \nonumber\\
			\nonumber\\
         &=& \sum_{i=1}^{k} \left\{ \alpha \left( T_i[t] - S_i[t-\upsilon] \right) \right.\nonumber\\
			& & + \left. \left(1 - \alpha \right) \left( L_i[t-1] + B_i[t-1] \right) \right\} \nonumber\\
         &=& \sum_{i=1}^{k} L_i[t] \label{equ:hw:l:pf}
\end{eqnarray}
\begin{eqnarray}
S^{*}[t] &=& \gamma (T^{*}[t] - L^{*}[t]         ) + (1 - \gamma) ( S^{*}[t-\upsilon]   ) \nonumber\\
         &=& \gamma \left[ \left(\sum_{i=1}^{k} T_i[t] \right) - \left( \sum_{i=1}^{k} L_i[t] \right) \right] \nonumber\\
         & & + (1 - \gamma) \left( \sum_{i=1}^{k} S_i[t-\upsilon]  \right) \textrm{~(by~(\ref{equ:hw:s:ih}), (\ref{equ:hw:l:pf}))} \nonumber\\
         &=& \sum_{i=1}^{k} \left\{ \gamma (T_i[t] - L_i[t] ) + (1 - \gamma) ( S_i[t-\upsilon] ) \right\} \nonumber\\
         &=& \sum_{i=1}^{k} S_i[t]
\end{eqnarray}
\end{proof}
%\vspace{-5pt}
\end{lem}



